Consistency of the posterior distribution in generalised linear inverse problems

For ill-posed inverse problems, a regularised solution can be interpreted as a mode of the posterior distribution in a Bayesian framework. This framework enriches the set the solutions, as other posterior estimates can be used as a solution to the inverse problem, such as the posterior mean that can be easier to compute in practice. In this paper we prove consistency of Bayesian solutions of an ill-posed linear inverse problem in the Ky Fan metric for a general class of likelihoods and prior distributions in a finite dimensional setting. This result can be applied to study infinite dimensional problems by letting the dimension of the unknown parameter grow to infinity which can be viewed as discretisation on a grid or spectral approximation of an infinite dimensional problem. Likelihood and the prior distribution are assumed to be in an exponential form that includes distributions from the exponential family, and to be differentiable. The observations can be dependent. No assumption of finite moments of observations, such as expected value or the variance, is necessary thus allowing for possibly non-regular likelihoods, and allowing for non-conjugate and improper priors. If the variance exists, it may be heteroscedastic, namely, it may depend on the unknown function. We observe quite a surprising phenomenon when applying our result to the spectral approximation framework where it is possible to achieve the parametric rate of convergence, i.e the problem becomes self-regularised. We also consider a particular case of the unknown parameter being on the boundary of the parameter set, and show that the rate of convergence in this case is faster than for an interior point parameter.

==> ChoiceOfDelta.tex <==

Condition (\ref{eq:LareDevIntegral}) is satisfied, for instance, under the following assumptions on $h_y$. Assume that  there exists a function $q>0$ such that for $x \in \X \setminus B(x^\star, \delta)$, $h_y(x) - h_y(x^\star) \geq  q(||x-x^\star||)$. Two types of behaviour of $q$ are considered.

1. Let  $q(r) \geq c r^{\alpha}$ for $r > \delta$ and some $c=c(\delta)>0,  \alpha \in(0,3)$.
Then, it is sufficient to choose $\delta $ satisfying
\begin{equation}\label{eq:CondDeltaLargeDev}
\int_{c\delta^\alpha/\tau}^{\infty} z^{p/\alpha -1} e^{-z} dz \ll  \alpha \tau^{-p/\alpha} c^{p/\alpha} \tau^{p_0/2+p_1/2}    (2\pi)^{p/2} [\det({H})]^{-1/2},
\end{equation}
which is satisfied, if $c(\delta) \asymp const$,
e.g. with  $\delta  = [-  \tau \log \tau]^{1/((1+a)\alpha)}$ for some $a>0$. In this case, it is possible to choose $\delta$ satisfying conditions (\ref{eq:CondDeltaLocal}) for appropriate $a$ and $\nu$ if $\alpha <3$.

Therefore, the following lemma holds.
\begin{lemma}\label{lem:LargeDev}
Assume that there exists a function $q: \, \mathbb{R}_+ \to \mathbb{R}_+ $ such that for $||x - x^\star||>\delta$, $h_y(x) - h_y(x^\star) \geq  q(||x-x^\star||)$, and   $q(r) \geq c r^{\alpha}$ for some $c=c(\delta)>0$ and $ \alpha \in (0,3)$.

Then, for $\delta$ satisfying Assumptions on $\delta$ stated in Section~\ref{sec:QuadraticApprox}, %(\ref{eq:CondDeltaLocal}) and  (\ref{eq:CondDeltaLargeDev}),
\begin{eqnarray*}
\int_{ \X} e^{- (h_y(x) - h_y(x^\star))/\tau} dx = [1+o(1)]\int_{B(x^\star, \delta)} e^{- (h_y(x) - h_y(x^\star))/\tau} dx
 \end{eqnarray*}
as $\tau \to 0$.

In particular, if $c(\delta) \asymp const$,  the above condition is satisfied with  $\delta  = [-  \tau \log \tau]^{1/((1+a)\alpha)}$ for any $a>0$.
\end{lemma}


2. If we assume that  $q(r) \geq c(\delta) \log r$  for $r>\delta$ and $c(\delta) > \tau (p+1)$, then
$$
\int_{ \X \setminus B(x^\star, \delta)} e^{- (h_y(x) - h_y(x^\star))/\tau} dx \leq C(p) \int_{r>\delta} r^{p-1 - c/\tau  } dr = \frac{C(p)}{c/\tau -p} \delta^{-c/\tau +p}.
$$
 To satisfy condition (\ref{eq:LareDevIntegral}) for small $\tau$, $\delta$ must satisfy
$$
%\delta^{c/\tau -p} (c/\tau -p) \gg \tilde{C}_H^{-1} \tau^{p_0/2} \gamma^{p_1 + 2p_2}
 c \delta^{c/\tau -p}  \gg \tilde{C}_H^{-1} \tau^{p_0/2+1} \gamma^{p_1 + 2p_2}
$$
for small $\tau$. This condition is satisfied if
$$
- c(\delta) \log \delta - \tau\log c(\delta) \ll - \tau \log \left(\tilde{C}_H^{-1} \tau^{p_0/2+1} \gamma^{p_1}  \right)
$$
with $\tilde{C}_H =  C_H / C(p)$, for instance, if $\delta$ is such that $-\log \delta \leq - C_1 \log(\tau \gamma)$ and $c(\delta) < C_2\tau$, for some $C_1, C_2>0$. If $c(\delta)$ is a constant independent of $\delta$, one of the conditions (\ref{eq:CondDeltaLocal}), that $\delta \to 0$, is not satisfied.
%  $c(\delta) = C \delta^{\alpha}$ for some $C,\alpha >0$


==> DataKyFan.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Convergence of the data in  Ky Fan metric}\label{sec:KyFanData}

Before giving the examples of application of Theorem~\ref{th:KyFanPostInt}, we consider some general inequalities for the Ky Fan distance.

\subsection{General inequalities}

%First, if $f_y(x)$ is regular enough, the first term in the upper
%bound on $\rho_{\rm P}(\mu_{\rm post}(\omega), \delta_{x^\star})$
%(Theorem \ref{th:ProkhUpperInt}) can be bounded in terms of the
%difference between data $y$ and the ``exact'' data $y_{y\exact}$
%(assumption 3 on the error distribution).

First we give upper bounds on the Ky Fan distance in terms of the moments of $||Y - \mu||$, and then consider particular cases with independent observations.

\begin{theorem}\label{th:KyFanMoments}
\begin{enumerate}

\item If $\exists \alpha >0$: \(\E e^{\alpha ||Y- \mu||} <\infty\), then
$$
\rho_{\rm K} (Y,\mu) \leq \E e^{\alpha ||Y- \mu||}.
$$

\item If $\exists \alpha >0$: \(\E \left[ ||Y- \mu||^{\alpha}\right] <\infty\), then
$$
\rho_{\rm K} (Y,\mu) \leq  \left[ \E ||Y- \mu||^{\alpha}\right]^{\frac 1 {1+\alpha}}.
$$
\end{enumerate}
\end{theorem}
The proof is obvious, applying the Markov inequality to the corresponding function of $||Y-\mu||$.

Now we evaluate the Ky Fan distance in the following two particular
cases:  the rescaled Poisson distribution, and  $Y_t = \mu_t +\sigma Z_t$ where the distribution of $Z_t$ is
independent of $\sigma$.



\subsection{Example}

We can see that the assumption of Corollary~\ref{eq:cor:KyFanRate} is satisfied not only for Gaussian random variables but also for  rescaled Poisson and binomial random variables.


% If $A^T V_{y\exact}(x^\star) A$ is not of full rank in  $P_0\X$, then we have the same rate as above.
%However, if $A^T V_{y\exact}(x^\star) A$ is of full rank in  $P_0\X$, then we have
%\begin{eqnarray*}
%\rho_{\rm K}(\mu_{\rm post}, \delta_{x^\star}) &\leqslant& C\max\left\{\sqrt{- \tau\log \tau},   -\gamma^2
%\log\left(\gamma^2   \right) (1+o(1))\right\}.
%\end{eqnarray*}


